Accurate Low-Degree Polynomial Approximation of Non-polynomial Operators for Fast Private Inference in Homomorphic Encryption

As machine learning (ML) permeates fields like healthcare, facial recognition, and blockchain, the need to protect sensitive data intensifies. Fully Homomorphic Encryption (FHE) allows inference on encrypted data, preserving the privacy of both data and the ML model. However, it slows down non-secure inference by up to five magnitudes, with a root cause of replacing non-polynomial operators (ReLU and MaxPooling) with high-degree Polynomial Approximated Function (PAF). We propose SmartPAF, a framework to replace non-polynomial operators with low-degree PAF and then recover the accuracy of PAF-approximated model through four techniques: (1) Coefficient Tuning (CT) -- adjust PAF coefficients based on the input distributions before training, (2) Progressive Approximation (PA) -- progressively replace one non-polynomial operator at a time followed by a fine-tuning, (3) Alternate Training (AT) -- alternate the training between PAFs and other linear operators in the decoupled manner, and (4) Dynamic Scale (DS) / Static Scale (SS) -- dynamically scale PAF input value within (-1, 1) in training, and fix the scale as the running max value in FHE deployment. The synergistic effect of CT, PA, AT, and DS/SS enables SmartPAF to enhance the accuracy of the various models approximated by PAFs with various low degrees under multiple datasets. For ResNet-18 under ImageNet-1k, the Pareto-frontier spotted by SmartPAF in latency-accuracy tradeoff space achieves 1.42x ~ 13.64x accuracy improvement and 6.79x ~ 14.9x speedup than prior works. Further, SmartPAF enables a 14-degree PAF (f1^2 g_1^2) to achieve 7.81x speedup compared to the 27-degree PAF obtained by minimax approximation with the same 69.4% post-replacement accuracy. Our code is available at https://github.com/EfficientFHE/SmartPAF.

==> src/00-abstract.tex <==
Machine learning (ML) is getting more pervasive. Wide adoption of ML in healthcare, facial recognition, and blockchain involves private and sensitive data. Inference on encrypted data, termed Fully Homomorphic Encryption (FHE), preserves the privacy of both data and the ML model. However, it slows down plaintext inference by six magnitudes, with a root cause of replacing non-polynomial operators with high-degree Polynomial Approximated Function (PAF).
To reduce the degree without sacrificing accuracy,
we propose (1) Coefficient Tuning (CT) to obtain a good initial coefficient value for each PAF, (2) Progressive Approximation (PA) to enable convergence by replacing non-polynomial operators and training parameters in a divide-and-conquer manner, and (3) Alternate Training (AT) to further improve the post-replacement accuracy. A combination of CT, PA, and AT enables the exploration of accuracy-latency space for FHE-domain ReLU replacement. Our evaluation shows that the optimal PAF with 14 degrees reduces 72\% latency compared to state-of-the-art 27-degree PAF with the same post-replacement accuracy (69.4\%) on ResNet-18 using ImageNet 1k dataset.

% with a deep chain of multiplication and bootstrapping.

% The latency overhead of privacy-preserving secure Machine Learning (ML) inference in the Fully Homomorphic Encryption (FHE) domain is dominated by the high-degree (27-degree) Polynomial Approximated Function (PAF) with a deep chain of FHE-based multiplication and bootstrapping. 
% Existing solutions replace ReLU with channel-wise fine-grain low-degree PAF, but cannot replace all ReLU functions or cannot guarantee convergence for PAF with higher than 5 degrees, rendering either prohibitive latency or severe accuracy degradation. To enable the exploration of the accuracy-latency tradeoff for PAF with different degrees, 

==> src/04-methodology.tex <==
\section{Experiment Methodology}
\label{sec:methodology}

In this section, we explain the methodology of experiments with corresponding metrics.

\subsection{Experiment Setup}
\subsubsection{Model, Benchmark and Dataset} 
The proposed technique was evaluated using ResNet-18, a model comprising 17 ReLU layers. ImageNet 1k, a widely used validation dataset in practical applications, was utilized for validation~\cite{resnet18, krizhevsky2012imagenet}. The dataset consists of 1000 training and 1000 validation images. Results from the technique applied to ResNet-18 on ImageNet 1k demonstrate its potential for transfer to other commonly used datasets with lower complexity, such as CIFAR-100, CIFAR-10, and MNIST.

\subsubsection{PAF Baseline} 
The main objective of this paper is to present novel training methods to mitigate the accuracy degradation in the ML model with ReLU replaced by PAF. To achieve this, we utilize initial coefficients from \cite{Lee2021PreciseAO} for composite polynomials with an overall degree greater than 14, as it has been established to result in optimal multiplication depth. Such PAFs are referred by the accuracy coefficient $\alpha$~\cite{Lee2021PreciseAO}. For composite polynomials with degrees less than 14, we adopt a method that leverages coefficients generation for $f_n$ and $g_m$ \cite{polynomial} to construct the composite polynomial $f_n\circ g_m$, where $m, n$ both represent the number of odd items in the polynomials, e.g. $f_n$ indicates a polynomial with $n+1$ odd items. We explore the constructed polynomial with post-replacement accuracy as the final metric with selected PAFs shown in \tabref{tab:PAF_baseline}. 

% we directly adopt the minimax approximated polynomial~\cite{Lee2021PreciseAO} to construct 14-degree (14 multiplication depth) and 27-degree (27 multiplication depth) composite polynomial and a different combination of building blocks PAF~\cite{polynomial} to construct further mixed polynomial composition with lower degree and multiplication depth. The baseline polynoimals are shown in \tabref{tab:PAF_baseline}, where the accuracy shown is the validation accuracy on ImageNet 1k after directly replacing ReLU in ResNet-18 with the corresponding PAF.

\begin{table*}[!htp]\centering
\caption{Baseline PAF and post-replacement validation accuracy}\label{tab:PAF_baseline}
\scriptsize
\resizebox{0.48\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}\hline
Form & $\alpha=10$ &$\alpha=7$ &$f_1^2 \circ g_1^2$ & $f_2\circ g_3$ & $f_2\circ g_2$ & $f_1\circ g_2$ \\\hline
Degree & 27 &14 &12 &12 &10 &8 \\
\makecell{Multiplication \\ Depth} & 29 &14 &12 &9 &8 &7 \\
Accuracy & 69.0 &64.7 &51.3 &49.4 &32 &18.6 \\
\hline
\end{tabular}}
\end{table*}


\subsubsection{Baseline Training Strategy}
\label{sec:baseline_training}
We choose a network-wise replacement and network-wise training as the baseline strategy adopted by most prior arts. The baseline training strategy involves replacing all ReLU functions with PAF, and fine-tuning all parameters of the ML model except for the coefficients of PAF with both Stochastic Weight Averaging (SWA) and dropout applied if accuracy could get benefits.\footnote{The original paper employs pretrained hyperparameters to fine-tune for 10 epochs with a learning rate that is dropped by $\frac{1}{10}$ at the 5th epoch. However, it does not disclose the specific values of the hyperparameters. Therefore, we tested and selected our own hyperparameters.} To ensure a fair comparison, all configurations are trained for the same number of epochs. In case there are remaining epochs after the completion of the techniques, the models will be continuously trained using the baseline strategy till the given number of epochs.

\subsubsection{Coefficient Tuning Setup}
To evaluate the performance of our proposed PAF, we construct a Coefficient Tuning dataset (CT dataset) based on the ImageNet 1k training dataset. The CT dataset is generated by collecting the input activations of each ReLU layer, along with their corresponding official output from ReLU as reference output. 90\% of the CT dataset is then randomly selected as the CT training dataset, with the remaining 10\% used as the validation dataset. For a given-degree approximated composite polynomial, the coefficients of PAF are fine-tuned for 40 epochs using an automatic scheduler to adaptively adjust the learning rate.

\subsubsection{Progressive Approximation and Alternate Training Setup}
\label{sec:PA_AT_Setup}
As for the evaluation of Progressive Approximation (PA) and Alternate Training (AT), we implement them on plaintext neural networks and evaluate their accuracy. To ensure a fair comparison, all configurations are trained for the same number of overall epochs. And the entire training is carried out step-by-step with a single step consisting of 20 epochs. The design point with the highest validation point within each step will be selected as the start point of the next step.

To further improve the accuracy, techniques such as Stochastic Weight Averaging (SWA) and dropout are applied, when deemed beneficial~\cite{SWA,dropout}. Even though different configurations may use different techniques at different epochs, the introduction of techniques still guarantees fairness without bias on different configurations. As such techniques only unleash the benefits for configurations with potential, for some configurations without such potential, even the introduction of both techniques cannot improve the accuracy. 

\subsubsection{CT+PA+AT Training Scheduler}
Different orders of applying PA and AT can affect the results.
We thus develop a custom scheduler to automatically manage the training flow. 
After each ReLU replacement, it trains the PAF coefficients and the parameters of other layers alternately with the same pertaining configurations. 
The scheduler chooses 20 epochs as a training group and changed policy in the granularity of training groups. Our scheduler applies dropout only once overfitting occurs together with a validation accuracy drop, and dropout will be added to the training configuration for the subsequent training. The training of a ReLU replacement will continue till the point no more accuracy improvement could be obtained, and the scheduler will start the replacement of the next ReLU.

% , the training configuration will change to train the parameters of layers except PAF and the corresponding default set, and the layers except PAF training follows the same flow. However, if there is no accuracy improvement during the group training, then the scheduler will replace the next ReLU layer and train it in the same way.

% and we thus construct a custom training scheduler to automatically apply PA and AT to the training as shown in~\figref{fig:flow_chart}. Note that the CT is applied offline before training, and it's thus not shown in the flow chart. The scheduler automatically manage the training flow.
% After each ReLU replacement, it will train PAF coefficients of the ReLU layer and the parameters of layers except PAF. alternately.  For different parameters training, it has the default training configurations as in table~\ref{tab:set_up}. 
% After replacement, the PAF coefficients are trained first. It will continuously be trained by 20 epochs as a group until there is no validation accuracy improvement. if overfit occurring causes the validation drop, it will add dropout to the training configuration, and continue training the layer. When there is no more accuracy improvement in the layer, the training configuration will be changed to train the parameters of layers except PAF and the corresponding default set, and the layers except PAF training follows the same flow. However, if there is no accuracy improvement during the group of training, then It will replace the next ReLU layer and train it in the same way.


\insertFigure{flow_chart}{Overview of training scheduler to leverage PA and AT.}

\subsubsection{Latency Evaluation}
The secure approximated Neural Network was implemented using the Microsoft SEAL library~\cite{SEAL}. Latency was measured by a single-threaded program compiled on an Intel 10750H CPU with 16 GB memory. The latency breakdown of ResNet-18 with the baseline FHE implementation shows that non-polynomial activation functions account for up to 18~\% of the overall latency.
\subsubsection{Accuracy Evaluation}
We obtain the validation accuracy of the plaintext-based neural network on the ImageNet 1k validation dataset because of the prohibitive latency of running FHE-based validation inference on the CPU to obtain the post-FHE accuracy, which is the same as our baseline implementation~\cite{Lee2021PreciseAO}. We report the highest validation accuracy during the training for all different training configurations. 

% and an NVIDIA RTX 2070 GPU with 8GB exclusive memory.

% collect the latency of deploying post-replacement polynomial approximation on the 
% Then all parameters except the coefficients in the PAF of the neural network get trained until the convergence of accuracy. 

